Quantum computing for data analysis in high energy physics

Some of the biggest achievements of the modern era of particle physics, such as the discovery of the Higgs boson, have been made possible by the tremendous effort in building and operating large-scale experiments like the Large Hadron Collider or the Tevatron. In these facilities, the ultimate theory to describe matter at the most fundamental level is constantly probed and verified. These experiments often produce large amounts of data that require storing, processing, and analysis techniques that often push the limits of traditional information processing schemes. Thus, the High-Energy Physics (HEP) field has benefited from advancements in information processing and the development of algorithms and tools for large datasets. More recently, quantum computing applications have been investigated in an effort to understand how the community can benefit from the advantages of quantum information science. In this manuscript, we provide an overview of the state-of-the-art applications of quantum computing to data analysis in HEP, discuss the challenges and opportunities in integrating these novel analysis techniques into a day-to-day analysis workflow, and whether there is potential for a quantum advantage.

==> Sections/VQCcircuit.tex <==
\begin{quantikz}
\lstick{$\ket{0}$} & \gate[wires=5]{U_{\phi}(\vec{x})}  & \gate[wires=5][2.0cm]{U_{rot}(\vec{\theta})} \gategroup[wires=5, steps=4, style={dashed, cap=round, fill=blue!20, inner ysep=20pt, inner xsep=70pt}, background, label style={label position=below, yshift=-0.5cm}]{repeat $l$ times}& \gate[wires=5][2.0cm]{U_{ent}} & \push{...} & \meter{}\rstick[wires=5]{labels $y$}\\
\lstick{$\ket{0}$} & {} & {} & {} & \push{...}& \meter{}\\
\lstick{$\ket{0}$} & {} & {} & {} & \push{...}& \meter{}\\
\lstick{$\vdots$}  & {} & {} & {} & \push{...}& \meter{}\\
\lstick{$\ket{0}$} & {} & {} & {} & \push{...}& \meter{}\\
\end{quantikz}

==> Sections/extra_text.tex <==
@article{Feynman1982,
  doi = {10.1007/bf02650179},
  url = {https://doi.org/10.1007/bf02650179},
  year = {1982},
  month = jun,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {21},
  number = {6-7},
  pages = {467--488},
  author = {Richard P. Feynman},
  title = {Simulating physics with computers},
  journal = {International Journal of Theoretical Physics}
}



==> Sections/info_processing.tex <==
\begin{itemize}
    \item Unfolding measurement distributions via quantum annealing \cite{Cormier2019}
\end{itemize}
